The Hubble Space Telescope UV Legacy Survey of Galactic Globular Clusters. XIII. ACS/WFC Parallel-Field Catalogues

As part of the Hubble Space Telescope UV Legacy Survey of Galactic Globular Clusters, 110 parallel fields were observed with the Wide Field Channel of the Advanced Camera for Surveys, in the outskirts of 48 globular clusters, plus the open cluster NGC 6791. Totalling about $0.3$ square degrees of observed sky, this is the largest homogeneous Hubble Space Telescope photometric survey of Galalctic globular clusters outskirts to date. In particular, two distinct pointings have been obtained for each target on average, all centred at about $6.5$ arcmin from the cluster centre, thus covering a mean area of about $23\,{\rm arcmin^{2}}$ for each globular cluster. For each field, at least one exposure in both F475W and F814W filters was collected. In this work, we publicly release the astrometric and photometric catalogues and the astrometrised atlases for each of these fields.

==> binhex.tex <==
%%
%% This is file `binhex.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% binhex.dtx  (with options: `style')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from binhex.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file binhex.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\edef\next{\toks0=%
   {\catcode`\noexpand\@=\the\catcode`\@\toks0{\the\toks0}}%
}
\next
\catcode`\@11
\def\next#1#2#3{\expandafter \def \csname bb@#1\endcsname##1%
  {#2\csname bb@#3##1\endcsname}}
\next{00}00 \next{01}01 \next{02}10 \next{03}11
\next{04}20 \next{05}21 \next{06}30 \next{07}31
\next{08}40 \next{09}41 \next{10}50 \next{11}51
\next{12}60 \next{13}61 \next{14}70 \next{15}71
\next{16}80 \next{17}81 \next{18}90 \next{19}91
\expandafter \def \csname bb@0+\endcsname {+0}
\expandafter \def \csname bb@1+\endcsname {+1}
\def\bb@endbinary#1+{\fi\fi}
\expandafter \def \csname bb@0-\endcsname {0+-\bb@dobinary}
\expandafter\def\csname bb@0m\endcsname#1+{#1+0}
\expandafter\def\csname bb@1m\endcsname#1+{#1+1}
\def\bb@dobinary#1#2{\if#10\if m\string#2\else\bb@endbinary\fi\fi
 \expandafter\bb@dobinary\number\csname bb@0#1\endcsname#2}
\def\nbinary#1#2{\expandafter\bb@dobinary\number\number#2%
 \romannumeral\number\number#1 000+}
\def\binary{\nbinary1}
\def \next #1#2{\expandafter \def
 \csname bb@h\number +#1\endcsname ##1+{\bb@dohex ##1+#2}%
}
\next   {0}0 \next   {1}1 \next  {10}2 \next  {11}3
\next {100}4 \next {101}5 \next {110}6 \next {111}7
\next{1000}8 \next{1001}9 \next{1010}A \next{1011}B
\next{1100}C \next{1101}D \next{1110}E \next{1111}F
\def\bb@dohex #1{\csname bb@x#1\endcsname}
\def\bb@x\endcsname#1{ \bb@xm{m\endcsname}}
\def\bb@xm #1\endcsname #2#3+{#2#3%
 \csname bb@h\number+\endcsname
 #1\endcsname m#3+}
\def\bb@nbinbased #1#2#3{\expandafter \bb@dobinary \number#1%
 \expandafter \bb@dohex
 \romannumeral \number\number #2 000\expandafter\endcsname
 \romannumeral \number\number #3 000+}
\def\nbinbased #1#2#3{\expandafter\bb@nbinbased
 \expandafter {\number#3}{#2}{#1}}
\def\nhex{\nbinbased4}
\def\noct{\nbinbased3}
\def\ntetra{\nbinbased2}
\def\hex{\nhex1}
\def\oct{\noct1}
\def\tetra{\ntetra1}
\the\toks0
\endinput
%%
%% End of file `binhex.tex'.

